Beyond Signal Propagation: Is Feature Diversity Necessary in Deep Neural Network Initialization?

Deep neural networks are typically initialized with random weights, with variances chosen to facilitate signal propagation and stable gradients. It is also believed that diversity of features is an important property of these initializations. We construct a deep convolutional network with identical features by initializing almost all the weights to $0$. The architecture also enables perfect signal propagation and stable gradients, and achieves high accuracy on standard benchmarks. This indicates that random, diverse initializations are \textit{not} necessary for training neural networks. An essential element in training this network is a mechanism of symmetry breaking; we study this phenomenon and find that standard GPU operations, which are non-deterministic, can serve as a sufficient source of symmetry breaking to enable training.

==> sections/LeakyNetRuns.tex <==

\renewcommand{\figscale}{2.1in}
\renewcommand{\figspacescale}{-0.1in}

\begin{figure*}[ht!]
    
    \centering
    \begin{subfigure}{}
        \centering
    	\includegraphics[width=3.00in]{figures/leakyNets/learkynet_forward_0.pdf}
    \end{subfigure}
    \begin{subfigure}{}
        \centering
    	\includegraphics[width=\figscale]{figures/leakyNets/learkynet_forward_20.pdf}
    \end{subfigure}
    \\
    \begin{subfigure}{}
        \centering
    	\includegraphics[width=\figscale]{figures/leakyNets/learkynet_forward_1.pdf}
    \end{subfigure}
    \hspace{\figspacescale}
    \begin{subfigure}{}
        \centering
    	\includegraphics[width=\figscale]{figures/leakyNets/learkynet_forward_2.pdf}
    \end{subfigure}
    \hspace{\figspacescale}
    \begin{subfigure}{}
        \centering
    	\includegraphics[width=\figscale]{figures/leakyNets/learkynet_forward_3.pdf}
    \end{subfigure}%
    \\
    \begin{subfigure}{}
        \centering
    	\includegraphics[width=\figscale]{figures/leakyNets/learkynet_forward_4.pdf}
    \end{subfigure}%
        \hspace{\figspacescale}
    \begin{subfigure}{}
        \centering
    	\includegraphics[width=\figscale]{figures/leakyNets/learkynet_forward_5.pdf}
    \end{subfigure}%
        \hspace{\figspacescale}
    \begin{subfigure}{}
        \centering
    	\includegraphics[width=\figscale]{figures/leakyNets/learkynet_forward_6.pdf}
    \end{subfigure}%
    \\
    \begin{subfigure}{}
        \centering
    	\includegraphics[width=\figscale]{figures/leakyNets/learkynet_forward_7.pdf}
    \end{subfigure}
    \hspace{\figspacescale}
    \begin{subfigure}{}
        \centering
    	\includegraphics[width=\figscale]{figures/leakyNets/learkynet_forward_8.pdf}
    \end{subfigure}
    \hspace{\figspacescale}
    \begin{subfigure}{}
        \centering
    	\includegraphics[width=\figscale]{figures/leakyNets/learkynet_forward_9.pdf}
    \end{subfigure}%
    \\
    \begin{subfigure}{}
        \centering
    	\includegraphics[width=\figscale]{figures/leakyNets/learkynet_forward_10.pdf}
    \end{subfigure}
    \hspace{\figspacescale}
    \begin{subfigure}{}
        \centering
    	\includegraphics[width=\figscale]{figures/leakyNets/learkynet_forward_11.pdf}
    \end{subfigure}
    \hspace{\figspacescale}
    \begin{subfigure}{}
        \centering
    	\includegraphics[width=\figscale]{figures/leakyNets/learkynet_forward_12.pdf}
    \end{subfigure}%
    \\
    \caption{The forward correlations of differently initialized leakyNets, during training. Average and error margin of two seeds per curve. Legend labels denote the number of identity initializations ('$I$') / number of average initializations ('$\mathbb{1}$'). Unlike what we saw in ConstNet, the correlations in leakyNets initialized with mixed '$I/\mathbb{1}$' do not converge to the same values seen in the case of i.i.d initialization (which eventually achieved higher test accuracy). }
    \label{fig:leakyNet_Correlations}
\end{figure*}

==> sections/group_behaviour.tex <==



\section{Mean field Theory of Symmetry Breaking}\label{sup:symBreak}

\subsection{Definitions}

When observing the values of an hidden layer $h \in \mathbb{R}^{c \times h_x \times h_y}$ as a result of some input $X$, we can define the correlation between the hidden states channels ($h^i \in \mathbb{R}^{h_x \times h_y},  0 \le i < c $) , as:

\begin{equation}\label{eq:HiddenLayerCorrelation}
    C_h \equiv \frac{1}{c\left(c-1\right)}\sum_{i}^{c}\sum_{i\ne j}^{c} \frac{h^{i}\cdot h^{j}}{\left\Vert h^{i}\right\Vert _{F}\left\Vert h^{j}\right\Vert _{F}}.
\end{equation}

In the exact same manner, as we consider the gradient of the loss $\mathcal{L}$ in respect to the hidden layer value, $g_i = \frac{d\mathcal{L}}{dH_i}, g_i \in \mathbb{R}^{h_x \times h_y}$, we can also define the \textit{gradient correlation}: 
\begin{equation}\label{eq:GradientCorrelation}
    C_g \equiv \frac{1}{c\left(c-1\right)}\sum_{i}^{c}\sum_{i\ne j}^{c} \frac{g^{i}\cdot g^{j}}{\left\Vert g^{i}\right\Vert _{F}\left\Vert g^{j}\right\Vert _{F}}.
\end{equation}

One additional component in the network that should be addressed before we move on is the activation function. Given activation function $\phi(x)$, and a normally distributed input $x_1,x_2\sim\mathcal{N}(0,\Sigma_{Q,C})$, $\Sigma_{Q,C}=Q\left(\begin{array}{cc}1 & C\\C & 1\end{array}\right)$ we can define the mapping function between the pre-activation correlation and the post activation output correlation:

\begin{align}\label{eq:activationMapping}
    \mathcal{M}_{Q}^{\phi}(Q) &\equiv \mathbb{E}_{x}\left[\phi^{2}(x_1)\right]\\
    \mathcal{M}^{\phi}(C) \equiv \mathcal{M}_{C}^{\phi}(C,Q) &\equiv  \frac{\mathbb{E}_{x}\left[\phi(x_{1})\phi(x_{2})\right]}{\mathbb{E}_{x}\left[\phi^{2}(x_1)\right]}
\end{align}

Note that $x$ distribution is defined using $Q,C$, and the dependency of $\mathcal{M}^{\phi}$ in $Q$ is implicit. We will denote the post activation tensor and it's gradient as $\ph, \pg$, and their correlations as $C_{\ph}, C_{\pg}$.
% \begin{align}\label{eq:activationMapping}
%     \mathcal{M}_{Q}(Q) &\equiv \int_{-\infty}^{\infty}\frac{1}{\sqrt{2\pi Q}}\exp\left[-\frac{x^{2}}{2Q}\right]\sigma^{2}(x)dx \\
%     \mathcal{M}_{C}(C,Q) &\equiv  \frac{1}{\mathcal{M}_{Q}(Q)}\int_{-\infty}^{\infty}\int_{-\infty}^{\infty}dx_{1}dx_{2}  ... 
% \end{align}

% \begin{equation*}
%      \frac{1}{2\pi Q\sqrt{1-C^{2}}} \cdot    \exp\left[-\frac{x_{1}^{2}-2Cx_{1}x_{2}+x_{2}^{2}}{2Q\left(1-C^{2}\right)}\right]\sigma(x_{1})\sigma(x_{2})
% \end{equation*}

\subsection{A Mean field Analysis of backward and forward correlations}\label{sup:meanfield_corrs}

Now that we have defined the relevant quantities for our analysis, we proceed in studying how those quantities effect each other, when considering a simple feed forward networks, composed of convolutions followed by a non-linear activation function. For simplicity, we will consider the simple case of fully-connected layer, where each input is regarded as a $1\times1$ channel, and rely on the analysis of \cite{xiao2018dynamical}, to deduce that the behaviour of each feasible Fourier mode of the convolution's weight filter will independently behave the same.

The first important observation, is that given some input $\ph^{(\ell)}$ (${\ell}$ superscript in this subsection will indicate the layer number) to a matrix-multiplication with the weight tensor $W^{(\ell)}$, the operation's output is $h^{(\ell)}= \ph^{(\ell)-1} W^{(\ell)}$. If we look at the different channels of the hidden layer, 
\begin{equation}\label{eq:output_formula}
    h_i^{(\ell)}= (\wout^i)^{(\ell)} \ph^{(\ell-1)}. 
\end{equation}
We note that each output channel is independent on the entire input tensor, but is only dependent on a single sub-tensor of the weights ($\wout^i$). To understand the correlation $C_h^L$, we apply the mean field technique, as seen in \cite{poole2016exponential,schoenholz2016deep,xiao2018dynamical}. However, we do not utilize this technique as was done in these papers: Previous papers studied the evolution of correlation between hidden layers resulted by different inputs, for a network initialized with normally distributed weights. Instead, we now look at the correlation between different channels, and assume, at first, that the layer-input and gradient is normally distributed. We will also take the mean field assumptions: our results will only be guaranteed to hold almost-surely in the limit where the number of input channels, output channels or the channel dimensions are taken to infinity.

Using the mean field technique over \ref{eq:output_formula}, we get $C_h^{(\ell)} = C_f^{(\ell)}$. Identical arguments can be used for the back-propagation as well: When considering the gradient of the post-activation hidden layer $\hat{g}$, we get that $C_{\hat{g}}^{(\ell)} = C_b^{(\ell+1)}$. We can use the result for propagation of covariance from \cite{schoenholz2016deep} to write the correlation of the pre-activation gradients as $C_g^{(\ell)} = C_{\pg}^{(\ell)}\mathcal{M}_{C}^{\phi'}(C_{h}^{(\ell)},Q)$, with $\phi'= \frac{\phi(x)}{dx}$. 

Next, we can use our newfound understanding of the inputs and gradients correlation to derive the correlation of the \textit{weight update}. When using standard gradient descent, our formula for the convolution $h^{(\ell)}=W^{(\ell)} \ph^{(\ell-1)}$ weights update is:
\begin{align}\label{eq:convUpdate}
    &\delta W^{(\ell)}=\eta\frac{d\mathcal{L}}{dW}=\eta\frac{d\mathcal{L}}{d\ph^{(\ell-1)}}\frac{d\ph^{(\ell-1)}}{dW^{(\ell)}}=\eta \ph^{(\ell-1)} g^{{(\ell)}} \\
    &(\delta\wout^{i})^{(\ell)}=\eta \ph^{(\ell-1)} (g^{i})^{{(\ell)}} \\
    &(\delta\win^{i})^{(\ell)}=\eta (\ph^{i})^{(\ell-1)} g^{{(\ell)}}
\end{align}

using this equations and the mean field technique from before, we learn that that the gradient updates correlations $\cdf^{(\ell)}, \cdb^{(\ell)} $ (of a single mode) also follow a simple relation in the mean field regime: 

\begin{align}\label{eq:updateCov}
    \cdf^{(\ell)} &= C_g^{(\ell)} = C_{\pg}^{(\ell)}\mathcal{M}_{C}^{\phi'}(C_{h}^{(\ell)}) = C_b^{(\ell+1)}\dMp(C_f^{(\ell)}) \\
    \cdb^{(\ell)} &= C_{\ph}^{(\ell-1)} = \Mp(C_{h}^{(\ell-1)}) =  \Mp(C_f^{(\ell-1)}) 
\end{align}

The equations we found for describing the relationship between correlations indicate of a "closed circle", rather than an evolution of the correlations through the layers, as seen in previous papers. Evidently, the forward correlation of the weights of one convolutional layer determines the backward correlation of the preceding layer's updates, and vice versa. We can therefore view the requirement to break symmetry in the neural network as the requirement to independently break all symmetries in numerous independent \textbf{groups}, each containing forward and backward correlations which affects one another.

When dealing with convolution, we are also required to do so for each distinct Fourier mode of the weight matrix, as these modes also act independently of one another.

This result could be extended to more complex models, with skip connection, where a group of more than two operations are directly connected to one another. In this case, the group may included several forward and backward correlations, affecting each other.

While the mean field assumption seems strict, the assumption regarding the inputs being normally distributed instigates a bigger problem. In models with symmetrical features as studied in our section \ref{sec:featureSym}, the inputs and gradients can be expected to be fully correlated, until the preceding layer has broken symmetry itself. This means, for once, that the behaviour of orthogonally initialized tensors is not captured well by this model: despite having a forward correlation of zero, orthogonal initialization will result correlated output when the input is correlated. 

\subsection{Evolution of correlations during training}\label{sup:evo_corr}

Having derived the forward/backward correlation between the weight updates, we would like to be able to describe the evolution of the gradients during training, in a single sub-network. To do so, we will start by simplifying the model, but taking additional assumptions: first, we will take an \textit{untied weights assumption}, that our updates at different steps of training are not correlated with each other. This assumption can be justified, for some degree, since both the input and the weights change in each step of training, as long as we remain close to the network initialization. We will also assume that the changes in the implicit variable $Q$ during training has been relatively small, allowing us to regard the activation function as fixed. Finally, we will treat the updates $\dwf, 
\dwb$ as if they are normally distributed: So for every weight update, $(\delta W)(t) \sim \mathcal{N}\left(\mu(t),\Sigma(t)\right)$, with $\Sigma(t)$ indicating $Q_{\delta}(t)$ variance, $C_{\delta f}(t)$ element-wise correlation between the $\wout$ sub-tensors' update and $C_{\delta b}(t)$ as the element wise correlation between the $\win$ sub-tensors' update. Using this model, we get

\begin{equation}\label{eq:correlationUpates}
    W=\sum_{i=0}^{T}(\delta W)^{i}\sim\mathcal{N}\left(\sum_{i=0}^{T}\mu_{i},\sum_{i=0}^{T}\left(\Sigma_{i}\right)\right).
\end{equation}

From this matrix, we can extract the backward and forward correlations:

\begin{align} 
Q_{\delta b}(T+1)=&\eta\mathcal{M^{\phi}}_{Q}(Q_{f}(T)) \\
Q_{\delta f}(T+1)=&\eta Q_{b}(T)\mathcal{M}_{Q}^{\phi'}(Q_{f}(T)) \\
Q_{f,b}(T+1)=&\sum_{t=0}^{T+1}Q_{\delta f,b}(t)=Q_{f,b}(T)+Q_{\delta f,b}(T+1) 
\end{align} 

when $Q_f,Q_b$ denotes the variances of the tensors corresponding to the correlations $C_f,C_b$ 

\begin{align} 
    &C_{f}(T+1)=\frac{\sum_{t=0}^{T+1}Q_{\delta f}(t)C_{\delta f}(t)}{\sum_{i=0}^{T+1}Q_{\delta f}(t)}=\\ %=\frac{1}{T}\sum_{i=0}^{T}C_{\delta f}(t) \\
    &\frac{Q_{f}(T)C_{f}(T)+Q_{\delta f}(T+1)C_{\delta f}(T+1)}{Q_{f}(T)+Q_{\delta f}(T+1)}=\\
    \label{eq:ForwardCorrelation}
    &\frac{Q_{f}(T)C_{f}(T)+Q_{\delta f}(T+1) C_{b}(T)\mathcal{M}^{\phi'}(C_{f}(T))}{Q_{f}(T)+Q_{\delta f}(T+1)}\\
    %=&\frac{T-1}{T}C_{f}(T-1)+ \frac1T\dMp(C_{b}(T-1)) \\ 
    &C_{b}(T+1)=\frac{\sum_{t=0}^{T+1}Q_{\delta f}(t)C_{\delta b}(t)}{\sum_{i=0}^{T+1}Q_{\delta b}(t)}= \\ \label{eq:BackwardCorrelation}
    &\frac{Q_{b}(T)C_{b}(T)+Q_{\delta b}(T+1)\mathcal{M}^{\phi}(C_{f}(T))}{Q_{b}(T)+Q_{\delta b}(T+1)}
\end{align}

For any fixed, stable value of $Q_{\delta} ~ Q(0)$  , the trivial condition for fixed point of this 2D system is $\Mp(C_f^{\star})=C_b^{\star}$, $C_b^{\star}\dMp(C_f^{\star})=C_f^{\star}$ or simply:

\begin{equation}\label{eq:correlationUpates}
    \dMp(C_f^{\star})\Mp(C_f^{\star}) = C_f^{\star}
\end{equation}

Since $\M(1)=1$ for all deterministic mappings, it is clear that $C_f^{\star}= C_b^{\star}=1$ is always a fixed point. To exit this fixed point, a symmetry breaking machenism is required. To check the of the fixed points stability, we will assume that $Q$ has stabilized so all values are identical, and we can take the derivative of eq. \ref{eq:ForwardCorrelation},\ref{eq:BackwardCorrelation}, and get:

\begin{align*} 
    \frac{dC_{f}(T)}{dC_{f}(T-1)}&=1-\frac1T(1-C_b(T)\M_f') \\
     \frac{dC_{f}(T)}{dC_{b}(T-1)}&= \frac1T \M_f \\
    \frac{dC_{b}(T)}{dC_{b}(T-1)}& = 1-\frac1T \\ 
    \frac{dC_{b}(T)}{dC_{f}(T-1)}&=\frac1T\M_b' 
\end{align*}

where $\frac{d}{dx} \M^{\phi'}(x) |_{x=C_{f}(T)} = \M_f', \frac{d}{dx} \M^{\phi}(x) |_{x=C_{f}(T)} = \M_b'$.
We get the jacobian
\begin{equation*}
J=\frac{1}{T}\left(\begin{array}{cc}
T-1\left(1-C_{b}(T)\mathcal{M}'_{f}\right) & \mathcal{M}_{f}\\
\mathcal{M}'_{b} & T-1
\end{array}\right)
\end{equation*}
with the eigenvalues:
\begin{equation}\label{eq:instability_condition}
    \lambda_{1,2}=1+\frac{1}{T}\left(\pm\sqrt{\frac{1}{4}\left(C_{b}\mathcal{M}'_{f}\right)^{2}+\mathcal{M}'_{b}\mathcal{M}_{f}}+\frac{1}{2}C_{b}\mathcal{M}'_{f}-1\right), 
\end{equation}
%%In our trivial fixed point, $C_b = \mathcal{M}_{b}$. 
In the fixed point itself, $C_b^{\star} = C_f^{\star} = 1$. The activation's mapping functions are convex, with fixed point at $\M(1)=1$ in case of deterministic activation function, so $\M_f=1$. We can now see that the fixed point at $c=1$ is unstable under the sufficient condition $\mathcal{M}'_{f}\ge1,\mathcal{M}'_{b}\ge 1$: 

\begin{equation}
    \lambda_{1}\ge1+\frac{1}{T}\left(\sqrt{\frac{1}{4}\left(1\right)^{2}+1}+\frac{1}{2}1-1\right)=1+\frac{1}{T}\left(\sqrt{\frac{5}{4}}-\frac{1}{2}\right)>1.
\end{equation}


Specifically for the ReLU activation,  $\lim_{C \to 1} {M}'_{b}(C) = \infty$, ensuring the instability of the fixed point when Relu is used.

% Our result indicate that the fixed point where features are correlated, becomes unstable under some trivial conditions for the activation function. In our model, the instability of the fixed point will decline as the training progress: 

%%so any fixed point will be stable, even without regarding the quickly diminishing $\frac1T$ term.
%We can see that in this case, and remember that $\Mp(c) < c$, the forward and backward correlations are remarkably stable: 






% As before, we will look at both the forward correlation and the backward correlation of the updates. 

% in the mean-field regime, the evolution of the correlation can best be described by observing each Fourier mode $\mathcal{F}[x]_{\alpha,\alpha'}$ individually, and consider each mode's respective correlation. For each input Fourier mode, 


==> sections/sg_symbreak.tex <==



\section{Mean field Theory of Symmetry Breaking}\label{sup:symBreak}



\subsection{Definitions}

When observing the values of an hidden layer $h \in \mathbb{R}^{c \times h_x \times h_y}$ as a result of some input $X$, we can define the correlation between the hidden states channels ($h^i \in \mathbb{R}^{h_x \times h_y},  0 \le i < c $) , as:

\begin{equation}\label{eq:HiddenLayerCorrelation}
    C_h \equiv \frac{1}{c\left(c-1\right)}\sum_{i}^{c}\sum_{i\ne j}^{c} \frac{h^{i}\cdot h^{j}}{\left\Vert h^{i}\right\Vert _{F}\left\Vert h^{j}\right\Vert _{F}}.
\end{equation}

In the exact same manner, as we consider the gradient of the loss $\mathcal{L}$ in respect to the hidden layer value, $g_i = \frac{d\mathcal{L}}{dH_i}, g_i \in \mathbb{R}^{h_x \times h_y}$, we can also define the \textit{gradient correlation}: 
\begin{equation}\label{eq:GradientCorrelation}
    C_g \equiv \frac{1}{c\left(c-1\right)}\sum_{i}^{c}\sum_{i\ne j}^{c} \frac{g^{i}\cdot g^{j}}{\left\Vert g^{i}\right\Vert _{F}\left\Vert g^{j}\right\Vert _{F}}.
\end{equation}

One additional component in the network that should be addressed before we move on is the activation function. Given activation function $\phi(x)$, and a normally distributed input $x_1,x_2\sim\mathcal{N}(0,\Sigma_{Q,C})$, $\Sigma_{Q,C}=Q\left(\begin{array}{cc}1 & C\\C & 1\end{array}\right)$ we can define the mapping function between the pre-activation correlation and the post activation output correlation:

\begin{align}\label{eq:activationMapping}
    \mathcal{M}_{Q}^{\phi}(Q) &\equiv \mathbb{E}_{x}\left[\phi^{2}(x_1)\right]\\
    \mathcal{M}^{\phi}(C) \equiv \mathcal{M}_{C}^{\phi}(C,Q) &\equiv  \frac{\mathbb{E}_{x}\left[\phi(x_{1})\phi(x_{2})\right]}{\mathbb{E}_{x}\left[\phi^{2}(x_1)\right]}
\end{align}

Note that $x$ distribution is defined using $Q,C$, and the dependency of $\mathcal{M}^{\phi}$ in $Q$ is implicit. We will denote the post activation tensor and it's gradient as $\ph, \pg$, and their correlations as $C_{\ph}, C_{\pg}$.
% \begin{align}\label{eq:activationMapping}
%     \mathcal{M}_{Q}(Q) &\equiv \int_{-\infty}^{\infty}\frac{1}{\sqrt{2\pi Q}}\exp\left[-\frac{x^{2}}{2Q}\right]\sigma^{2}(x)dx \\
%     \mathcal{M}_{C}(C,Q) &\equiv  \frac{1}{\mathcal{M}_{Q}(Q)}\int_{-\infty}^{\infty}\int_{-\infty}^{\infty}dx_{1}dx_{2}  ... 
% \end{align}

% \begin{equation*}
%      \frac{1}{2\pi Q\sqrt{1-C^{2}}} \cdot    \exp\left[-\frac{x_{1}^{2}-2Cx_{1}x_{2}+x_{2}^{2}}{2Q\left(1-C^{2}\right)}\right]\sigma(x_{1})\sigma(x_{2})
% \end{equation*}

\subsection{Breaking symmetry in subgroups}\label{sup:meanfield_corrs}
Now that we have defined the forward and backward correlations, we can proceed in studying how those quantities effect each other, when considering a simple feed forward networks, composed of convolutions followed by a non-linear activation function. For simplicity, we will consider the simple case of fully-connected layer, where each input is regarded as a $1\times1$ channel, and rely on the analysis of \cite{xiao2018dynamical}, to deduce that the behaviour of each feasible Fourier mode of the convolution's weight filter will independently behave the same.

The first important observation, is that given some input $\ph^{(\ell)}$ (${\ell}$ superscript in this subsection will indicate the layer number) to a matrix-multiplication with the weight tensor $W^{(\ell)}$, the operation's output is $h^{(\ell)}= \ph^{(\ell)-1} W^{(\ell)}$. If we look at the different channels of the hidden layer, 
\begin{equation}\label{eq:output_formula}
    h_i^{(\ell)}= (\wout^i)^{(\ell)} \ph^{(\ell-1)}. 
\end{equation}
We note that each output channel is independent on the entire input tensor, but is only dependent on a single sub-tensor of the weights ($\wout^i$). To understand the correlation $C_h^L$, we apply the mean field technique, as seen in \cite{poole2016exponential,schoenholz2016deep,xiao2018dynamical}. However, we do not utilize this technique as was done in these papers: Previous papers studied the evolution of correlation between hidden layers resulted by different inputs, for a network initialized with normally distributed weights. Instead, we now look at the correlation between different channels, and assume, at first, that the layer-input and gradient is normally distributed. We will also take the mean field assumptions: our results will only be guaranteed to hold almost-surely in the limit where the number of input channels, output channels or the channel dimensions are taken to infinity.

Using the mean field technique over \ref{eq:output_formula}, we get $C_h^{(\ell)} = C_f^{(\ell)}$. Identical arguments can be used for the back-propagation as well: When considering the gradient of the post-activation hidden layer $\hat{g}$, we get that $C_{\hat{g}}^{(\ell)} = C_b^{(\ell+1)}$. We can use the result for propagation of covariance from \cite{schoenholz2016deep} to write the correlation of the pre-activation gradients as $C_g^{(\ell)} = C_{\pg}^{(\ell)}\mathcal{M}_{C}^{\phi'}(C_{h}^{(\ell)},Q)$, with $\phi'= \frac{\phi(x)}{dx}$. 

Next, we can use our newfound understanding of the inputs and gradients correlation to derive the correlation of the \textit{weight update}. When using standard gradient descent, our formula for the convolution $h^{(\ell)}=W^{(\ell)} \ph^{(\ell-1)}$ weights update is:

\begin{align}\label{eq:convUpdate}
    &\delta W^{(\ell)}=\eta\frac{d\mathcal{L}}{dW}=\eta\frac{d\mathcal{L}}{d\ph^{(\ell-1)}}\frac{d\ph^{(\ell-1)}}{dW^{(\ell)}}=\eta \ph^{(\ell-1)} g^{{(\ell)}} \\
    &(\delta\wout^{i})^{(\ell)}=\eta \ph^{(\ell-1)} (g^{i})^{{(\ell)}} \\
    &(\delta\win^{i})^{(\ell)}=\eta (\ph^{i})^{(\ell-1)} g^{{(\ell)}}
\end{align}

using this equations and the mean field technique from before, we learn that that the gradient updates correlations $\cdf^{(\ell)}, \cdb^{(\ell)} $ (of a single mode) also follow a simple relation in the mean field regime: 

\begin{align}\label{eq:updateCov}
    \cdf^{(\ell)} &= C_g^{(\ell)} = C_{\pg}^{(\ell)}\mathcal{M}_{C}^{\phi'}(C_{h}^{(\ell)}) = C_b^{(\ell+1)}\dMp(C_f^{(\ell)}) \\
    \cdb^{(\ell)} &= C_{\ph}^{(\ell-1)} = \Mp(C_{h}^{(\ell-1)}) =  \Mp(C_f^{(\ell-1)}) 
\end{align}

The equations we found for describing the relationship between correlations indicate of a "closed circle", rather than an evolution of the correlations through the layers, as seen in previous papers. Evidently, the forward correlation of the weights of one convolutional layer determines the backward correlation of the preceding layer's updates, and vice versa. We can therefore view the requirement to break symmetry in the neural network as the requirement to independently break all symmetries in numerous independent \textbf{subgroups}, each containing forward and backward correlations which affects one another.

When dealing with convolution, we are also required to do so for each distinct Fourier mode of the weight matrix, as these modes also act independently of one another.

This result could be extended to more complex models, with skip connection, where a group of more than two operations are directly connected to one another. In this case, the subgroup may included several forward and backward correlations, affecting each other.

While the mean field assumption seems strict, the assumption regarding the inputs being normally distributed instigates a bigger problem. In models with symmetrical features as studied in our section \ref{sec:featureSym}, the inputs and gradients can be expected to be fully correlated, until the preceding layer has broken symmetry itself. This means, for once, that the behaviour of orthogonally initialized tensors is not captured well by this model: despite having a forward correlation of zero, orthogonal initialization will result correlated output when the input is correlated. 


% Our result indicate that the fixed point where features are correlated, becomes unstable under some trivial conditions for the activation function. In our model, the instability of the fixed point will decline as the training progress: 

%%so any fixed point will be stable, even without regarding the quickly diminishing $\frac1T$ term.
%We can see that in this case, and remember that $\Mp(c) < c$, the forward and backward correlations are remarkably stable: 






% As before, we will look at both the forward correlation and the backward correlation of the updates. 

% in the mean-field regime, the evolution of the correlation can best be described by observing each Fourier mode $\mathcal{F}[x]_{\alpha,\alpha'}$ individually, and consider each mode's respective correlation. For each input Fourier mode, 


==> tables/constnet_tbl.tex <==




\begin{table}[t]
\begin{center}
\begin{tabular}{| c  | c | c  | c |}
\hline
Model           & Init            & Variation         &  Acc[\%]   \\ [1.0ex]
\hline
Wide-ResNet     & He              &  Learning rate: $0.1$       &         95.51          \\ [1ex] 
\hline
%%Wide-ResNet     & He              &  --              &       95.33      \\ [1ex] 
%%\hline
ConstNet        & He             &  --    &         $94.85\pm0.06$         \\ [1ex] 
% results: 94.81, 94.89
\hline
ConstNet        & $0$             &  --              &       $94.78\pm0.06$ \\ [1ex] 
% results: 94.82, 94.73
\hline
ConstNet        & $0$             & Deterministic            &     \red{24.73}             \\ [1ex] 
\hline
ConstNet        & $0$             & \makecell{1\% Dropout \\  Deterministic}    &   $94.12\pm0.08$     \\ [1ex] 
\hline
% results: 94.18, 94.06
%ConstNet        & $0$             & Partial BN + Tune*    &   95.73     \\ [1ex] 
%\hline




\end{tabular}
\end{center}
\caption{Experiment results (Test Accuracy) of training a ConstNet over the CIFAR10 dataset. Despite starting from all-identical features ('$0$'-Init), a minimal mechanism of symmetry breaking is sufficient for ConstNet to train. }
%*Tune- This result was obtained by grid search of Mixup parameter and learning rate. }
\label{tbl:constnet_results}
\end{table}



==> tables/leakynet_results.tex <==




\begin{table}[h!]
\begin{center}
 \begin{tabular}{| c | c | c | c | c  | c|}
 \hline
Model & \multicolumn{4}{c|}{Init (Number of Layers)} & Acc[\%] \\ [1.0ex]
 \cline{2-5}
          &   Total  &     He   &    '$I$'    &   '$\mathbb{1}$'     &                \\ [1.0ex]
\hline 
LeakyNet     & 12  &   12      &      -        &    -       &     95.72      \\ [1ex] 
\hline
LeakyNet     & 12  &   -      &      12        &    -       &     94.87      \\ [1ex] 
\hline
LeakyNet     & 12  &   -      &      10        &    2       &    94.58    \\ [1ex] 
\hline
LeakyNet     & 12  &   -      &      8        &    4       &     88.44    \\ [1ex] 
\hline
LeakyNet     & 12  &   -      &      6        &    6       &   \orange{51.56}   \\ [1ex] 
\hline
LeakyNet     & 12  &   -      &      -        &    12       &     \red{33.98}      \\ [1ex] 
\hline

\end{tabular}
\end{center}
\caption{ Experiment results (Test Accuracy) of training a LeakyNet over the CIFAR10 dataset.} 
\label{tbl:leakynet_results}
\end{table}




% \begin{table}[!b]
% \begin{center}
%  \begin{tabular}{| c || c | c | c  || c|}
%  \hline
% Model & \multicolumn{4}{c||}{Initialization (# of Layers)} & Acc[\%] \\ [1.0ex]
%  \cline{2-5}
%           &   Total  &     He   &    'i'    &   '1'     &                \\ [1.0ex]
%  \hline\hline
% 0.01      &\xmark     &\xmark     &\xmark     & \xmark    & 95.2  \\ [1ex] 
% \hline
% 0.15      &\checkmark &\checkmark &\xmark     & \xmark    & 95.5 \\ [1ex] 
% \hline
% 0.1       &\checkmark &\checkmark &\checkmark & \xmark    & 95.3  \\ [1ex] 
% \hline
% 0.01      &\checkmark &\checkmark &\checkmark & \xmark    & 95.3  \\ [1ex] 
% \hline
% 0.00      &\checkmark &\checkmark &\checkmark & \xmark    & 95.0  \\ [1ex] 
% \hline
% 0.1       &\checkmark &\checkmark &\checkmark & \checkmark& 95.2    \\ [1ex] 
% \hline
% 0.01      &\checkmark &\checkmark &\checkmark & \checkmark& 95.3    \\ [1ex] 
% \hline
% 0.00      &\checkmark &\checkmark &\checkmark & \checkmark& 10.0*     \\ [1ex] 
% \hline
%  \hline
% \end{tabular}
% \end{center}
% \caption{Results of training a Resnet-like network with varying initializations and drop-rates after 200 epochs. The different initialization parts are: (a) Whether the weights on the convolution in the residual blocks is set to zero. (b) Whether the final FC layer weights are set to zero. (c) Whether the initial convolution is symmetrical and constant for all input and output channels. (d) Whether the weights of the $(1,1)$ convolutions used to adjust the dimensions when widening the residual blocks is initialized with a single constant. *Non-deterministic GPU computations (which are the default when using the NVIDIA cuDNN library) enable training with (a-d) enabled and \textit{no dropout}, leading to similar performance to a standard random initialization.%*The column "Robust" is marked with \xmark \space if runs without visible training in the first 5 epochs were observed: in this case, the unsuccessful runs were immediately discarded. This phenomena can be avoided by using a lower learning rate ($< 0.03$).
% }
% \label{tbl:constnet_results}
% \end{table}

==> tables/symbreaking_table.tex <==



\begin{table}[b!]
\begin{center}
 \begin{tabular}{| c | c | c | c | c| c|}
 \hline
Hardware           & Data-type & \makecell{Computation \\ Noise}  & \multicolumn{3}{c|}{\makecell{Drop Rate:}\vspace{-0.3cm}}  \\ [1.0ex]
 \cline{4-6}
                   &           &                 &   $0\%$        &   $0.1\%$ &   $1\%$   \\ [1.0ex]
                   
 \hline
GeForce GTX-1080  & FP32       &        \cmark   &   \green{*94.09\% }      &   \green{94.83\%} &  \green{*94.8\%}  \\ 
 \hline
GeForce GTX-1080  & FP32       &        \xmark   &   \red{24.96\%}      &   \orange{92.72\%} &  \orange{92.99\%}  \\ 
 \hline
GeForce RTX-2080  & FP32       &        \cmark   &   \red{*77.81\%}      &   \green{94.64\%} &  \green{95.05\%}  \\
\hline
GeForce RTX-2080  & FP32       &        \xmark   &   \red{24.80\%}      &   \orange{92.69\%} &  \orange{92.58\%}  \\ 
\hline
GeForce RTX-2080  & FP16       &        \cmark   &   \red{38.61\%}      &   \green{94.58\%} &  \green{94.62\%}  \\ 
 \hline
GeForce RTX-2080  & FP16       &        \xmark   &   \red{22.55\%}      &   \orange{91.99\%} &  \orange{92.55\%}  \\ 
 \hline

\end{tabular}
\end{center}
\caption{Experiment results (Test Accuracy) of training a ConstNet over the CIFAR10 dataset, with 200 epochs, $0$ initialization ensuring identical features, and varying symmetry-breaking mechanisms. Number of seeds of the different results vary. Dropout/ Computation noise by themselves are insufficient for successful training: the symmetry breaking in this case is too slow, and it come in the expense of the training process. Additionally, we can see a big gap between the effects of computation noise of different GPUs. When utilizing a 16-bit floating-point hardware architecture for a FP16 model, the hardware noise is insufficient and the training fails. *This result expanded upon in more details in Appendix \ref{sup:lim}.}
%*Tune- This result was obtained by grid search of Mixup parameter and learning rate. }
\label{tbl:symbreaking_comparison}
\end{table}

% GeForce GTX-1080
% constnet_a0_cudnn_dropout_001_A: 95.01
% constnet_a0_cudnn_dropout_01_A: 94.83
% constnet_a0_cudnn_dropout_0_A: 94.64

% constnet_a0_dropout_001_A: 92.72
% constnet_a0_dropout_01_A: 92.99
% constnet_a0_dropout_0_A: 23.96

% GeForce RTX-2080

% constnet_a0_cudnn_dropout_001_A: 94.64
% constnet_a0_cudnn_dropout_01_A: 95.05
% constnet_a0_cudnn_dropout_0_A: 94.64

% constnet_a0_dropout_001_A: 92.69
% constnet_a0_dropout_01_A: 92.58
% constnet_a0_dropout_0_A: 23.80

% constnet_a0_fp16_cudnn_dropout_001_A: 94.58
% constnet_a0_fp16_cudnn_dropout_01_A: 94.62
% constnet_a0_fp16_cudnn_dropout_0_A: 38.61

% constnet_a0_fp16_dropout_001_A: 91.99
% constnet_a0_fp16_dropout_01_A: 92.55
% constnet_a0_fp16_dropout_0_A: 22.55
